An Automated Deployment and Testing Framework for Resilient Distributed Smart Grid Applications

Executing distributed cyber-physical software processes on edge devices that maintains the resiliency of the overall system while adhering to resource constraints is quite a challenging trade-off to consider for developers. Current approaches do not solve this problem of deploying software components to devices in a way that satisfies different resilience requirements that can be encoded by developers at design time. This paper introduces a resilient deployment framework that can achieve that by accepting user-defined constraints to optimize redundancy or cost for a given application deployment. Experiments with a microgrid energy management application developed using a decentralized software platform show that the deployment configuration can play an important role in enhancing the resilience capabilities of distributed applications as well as reducing the resource demands on individual nodes even without modifying the control logic.

==> behaviormodel.tex <==
py 'starting test'
py time.sleep(1200)
py 'link failure'
py time.time()
link s1 h2 down
py time.sleep(1200)
py 'starting attack'
h7 xterm -T h7 -e python3 Attacker.py
py time.sleep(300)
py 'end of test'
py 'end'

==> hwspec.tex <==
# Specifications for the embedded nodes

#Beaglebone Black

[bbb]
# no. of CPU cores
cores = 1
max\_cpu = 0.7
# Internal memory (mb)
mem = 512
max\_mem = 0.7
# disk space (mb)
spc = 4096
max\_spc = 0.7

# network switch specifications
[generic\_switch]
# no. of ports
ports = 12
# speed in Mbps by port
speeds = 1024
#full duplex capability (optional)
#full\_duplex = true

==> remapp.tex <==
// RIAPS Energy management app

app REMApp {

message ChargerQry; 	// Query to charger interface
message ChargerAns;		// Answer from charger interface; (Current Power, number of sessions, the charged energy for each session)
message ChargerCmd;		// Command to charger (to set power); (Sessions to end if shed load)
message ChargerAck;		// Ack message
message ChargerUpdateData;  //Data send to predictive model
message ChargerPrediction;  //Prediction send back to manager

message BuildingQry;	// Query to building interface
message BuildingAns; 	// Answer from building interface (Current Power, Outside Air Temperature, HVAC power, Current Indoor Sensor Temperature)
message BuildingCmd;	// Command to charger (to set power) (Temperature offset)
message BuildingAck;	// Ack message
message BuildingUpdateData;  //Data send to predictive model
message BuildingPrediction;  //Prediction send back to manager

message BESSQry;	// Query to BESS interface
message BESSAns; 	// Answer from BESS interface (Current Power, Outside Air Temperature, HVAC power, Current Indoor Sensor Temperature)
message BESSCmd;	// Command to charger (to set power) (Temperature offset)
message BESSAck;	// Ack message

message PowerRequest; 		// Predicted load+flexbility (Predicted power for the next interval, available load shedding capacity for the next interval for each building, flexbility for each EV charging session)
message PowerDispatched;

message GridPower;		// Grid power (Available grid power for the next interval)
message GridCmd;
message LogData;
message EventData;
message EventLog;
message LogDataInternal;

message BuildingManagerGroupMsg;
message ChargerManagerGroupMsg;
message BESSManagerGroupMsg;
message CoordinatorGroupMsg;

message FDIACtrl;

group BuildingManagerGroup with leader using BuildingManagerGroupMsg;
group ChargerManagerGroup with leader using ChargerManagerGroupMsg;
group BESSManagerGroup with leader using BESSManagerGroupMsg;
group CoordinatorGroup with leader using CoordinatorGroupMsg;

library config;
library models;

//////////////######Components for Charger######///////////
// Device interface to charger system
device ChargerInterface(configfile) {
  inside relay; 							// inside port	
  ans request : (ChargerQry, ChargerAns);	// query from manager
  ans command : (ChargerCmd, ChargerAck);	// commands from manager
  sub FDIACmd: FDIACtrl ;
}

//device to house predictive model
device ChargerPredictive(model_path){
 ans updateAndPredict: (ChargerUpdateData,ChargerPrediction);
}

device Attacker(port) {
	pub sendFDIACmd : FDIACtrl ;
	inside trigger;
}

// Manager for charger system
component ChargerManager(id, grptype) {
  timer trigger 300 sec;						// timer to trigger a query on interface
  qry poller: (ChargerQry, ChargerAns);		// query to interface
  qry command: (ChargerCmd, ChargerAck);	// command to interface
  qry updateAndPredict:(ChargerUpdateData,ChargerPrediction);  //added query port for predictive model device
  pub reqPower: PowerRequest;					// predicted load
  sub dspPower: PowerDispatched;
  pub eventData : EventData;
  timer tick;
  timer votetrigger;
  sub FDIACmd: FDIACtrl ;
}


//////////////######Components for Building######///////////
// Device interface to building system
device BuildingInterface(configfile) {
  inside relay;								// inside port
  ans request : (BuildingQry, BuildingAns);	// queries from manager
  ans command : (BuildingCmd, BuildingAck);	// commands from manager
}

//device to house predictive model
device BuildingPredictive(model_path){
 ans updateAndPredict: (BuildingUpdateData,BuildingPrediction);
}

// Manager for building system
component BuildingManager(id, grptype) {
  timer trigger 300 sec;						// timer to trigger a query on interface
  qry poller : (BuildingQry, BuildingAns);	// query to interface
  qry command: (BuildingCmd, BuildingAck);	// command to interface
  qry updateAndPredict:(BuildingUpdateData,BuildingPrediction);  //added query port for predictive model device
  pub reqPower: PowerRequest;					// predicted load
  sub dspPower: PowerDispatched;
  pub eventData: EventData;
  timer tick;
  timer votetrigger;
}

//////////////######Components for BESS######///////////
// Device modeling a BESS
device BESS(Rbess,Cbattery,SoCl,SoCu,SoC0,SoCend,tStart,Ts) {
  inside relay;								// inside port
  ans request : (BESSQry, BESSAns);	// queries from manager
  ans command : (BESSCmd, BESSAck);	// commands from manager
}


// Manager for BESS
component BESSManager(id, grptype) {
  timer trigger 300 sec;						// timer to trigger a query on interface
  qry poller : (BESSQry, BESSAns);	// query to interface
  qry command: (BESSCmd, BESSAck);	// command to interface
  pub reqPower: PowerRequest;					// predicted load
  sub dspPower: PowerDispatched;
  pub eventData: EventData;
  timer tick;
  timer actuatetrigger;
  timer votetrigger;
}


device Grid(endpoint) {
  inside trigger;
  timer clock 300 sec;					// life signal
  timer ticker 75 sec;					// timer to send out grid power
  pub setPoint : GridCmd; 					// available power from grid
}

component GridManager() {
	sub setPoint : GridCmd;
	pub power : GridPower;
	pub eventData : EventData;
}

component Coordinator(configfile, id, grptype) {
   sub power: GridPower;				// available power from grid
   sub reqPower : PowerRequest;				// predicted load
   pub dspPower: PowerDispatched; 
   pub logData : LogData;
   pub eventData : EventData;
   timer tick; 
}

// Logger
component Logger(configfile) {
	sub logData : LogData;
	sub eventData : EventData;
	pub eventLog : EventLog;
	pub logDataInternal : LogDataInternal;
}

device LoggerInternal(configfile) {
	sub logDataInternal : LogDataInternal;
}

device EventLogger(configfile) {
	sub eventLog : EventLog;
	timer update 1 sec;
}

actor ChargerActor(id, grptype, configfile, model_path, port) {
	
   local ChargerQry, ChargerAns, ChargerCmd, ChargerAck, ChargerUpdateData, ChargerPrediction, FDIACtrl;
   uses {
			// cpu max 30 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			 // space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits 
		}
   {
	charger : ChargerInterface(configfile = configfile);
	manager : ChargerManager(id=id, grptype=grptype);
    predictive : ChargerPredictive(model_path = model_path);
    attacker: Attacker(port=port);
   }
}

actor BuildingActor(id, grptype, configfile, model_path) {
   local BuildingQry, BuildingAns, BuildingCmd, BuildingAck, BuildingUpdateData, BuildingPrediction;
   uses {
			//cpu max 30 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			// space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits
		}
   {
	building : BuildingInterface(configfile = configfile);
	manager : BuildingManager(id=id, grptype=grptype);
	predictive : BuildingPredictive(model_path = model_path);	
   }
}

actor BESSActor(id, grptype, Rbess,Cbattery,SoCl,SoCu,SoC0,SoCend,tStart='',Ts=60) {
   local BESSQry, BESSAns, BESSCmd, BESSAck;
   uses {
			//cpu max 30 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			// space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits
		}
   {
	bess : BESS(Rbess = Rbess,Cbattery=Cbattery,SoCl=SoCl,SoCu=SoCu,SoC0=SoC0,SoCend=SoCend,tStart=tStart,Ts=Ts);
	manager : BESSManager(id=id, grptype=grptype);	
   }
}

actor Aggregator(configfile, id, grptype) {
	   uses {
			// cpu max 35 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			// space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits
		}
   {
	coordinator : Coordinator(configfile=configfile, id= id, grptype=grptype);
   }
 }
 
actor DataLogger(configfile1, configfile2) {
	local EventLog, LogDataInternal;
	uses {
			// cpu max 25 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			// space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits
		}
   {
	logger: Logger(configfile=configfile1);
	logdataint : LoggerInternal(configfile=configfile1);
	eventlogger : EventLogger(configfile = configfile2);
   }
 }
 
actor UtilityGrid(endpoint) {
	local GridCmd;
	uses {
			// cpu max 25 % over 1;		// Hard limit, w/o 'max' = soft limit
			// mem 200 mb;					// Mem limit
			// space 2048 mb;				// File space limit
			net rate 40 kbps ceil 60 kbps burst 12 k; // Net limits
		}
   {
	grid : Grid(endpoint = endpoint);
	manager : GridManager();
   }
 }

}



==> remappfinal.tex <==

app REMApp {
    on (h1) BuildingActor() ;
    on (h1) DataLogger() ;
    on (h1) UtilityGrid() ;
    on (h2) Aggregator() ;
    on (h2) BuildingActor() ;
    on (h3) BESSActor() ;
    on (h4) BESSActor() ;
    on (h5) ChargerActor() ;
    on (h6) BESSActor() ;
    on (h7) ChargerActor() ;
    on (h8) Aggregator) ;
    on (h8) BuildingActor() ;
    on (h9) ChargerActor() ;
    }
        

==> riapsoverview.tex <==
\section{RIAPS Overview}
\label{riapsoverview}

The \textit{Resilient Information Architecture Platform for Smart Grids (RIAPS)} \cite{ghosh2019design} is an integrated, decentralized software framework that can be used for the development, deployment, and monitoring of distributed applications on remote hardware nodes, called RIAPS nodes. It supports a distributed model of computation where a user can define actors containing a number of \verb+components+ that run different computations and can communicate with each other via message passing through interfaces called \verb+ports+. On top of it, it also provides a number of platform services for remote node control, coordination, fault monitoring, time synchronization and so on.  Figure \ref{fig_riaps} depicts the RIAPS infrastructure . Interested readers can refer to \cite{ghosh2019design} for a detailed description of the RIAPS architecture and features. A RIAPS application is represented by an \texttt{app.riaps} file that describes the actor-component relationships along with the various message types and communication ports that each component uses. It also has an associated deployment file, \texttt{app.depl}, where the assignment of the actors to target computing nodes is specified.


% It is a completely distributed run-time software environment that supports real-time communication between the computing nodes, called "RIAPS nodes", and manages the deployment and execution of actors on these remote nodes. It also supports a completely distributed model of computation in which application functions are realized through message passing and event based logic among distributed software components. 

%  In RIAPS, the unit of computation with respect to fault tolerance is an actor that runs as a separate process within its own address space. The distributed applications are formed from actors that consist of multiple \texttt{components} that interact with each other only via messages. Components realize specific functions as designed by the application developer. Components can be implemented as Python or C++ classes. RIAPS also supports specialized components called \texttt{device components} that can be used to interface with physical hardware devices such as relays or sensors. RIAPS provides the underlying messaging framework for the components through interfaces called \texttt{ports} with \verb+send+ and \verb+receive+ operations, which can support a variety of communication patterns. It also provides a suite of out of the box services such as administration and control of the distributed application (from a control node), network discovery, time synchronization, platform level fault detection and recovery, dynamic logical grouping of components and coordinated actions and so on. This separates the business logic of the application from the low-level framework details. Figure \ref{fig_riaps} depicts the RIAPS infrastructure . Interested readers can refer to \cite{ghosh2019design} for a detailed description of the RIAPS architecture and features.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{figures/infrastructure.jpg}
\caption{RIAPS Network showing the RIAPS nodes, actors and components and the various services (some)}
\label{fig_riaps}
\end{figure}

==> tables/basic12node.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{l|l|l|l|l|l|l|}
\cline{2-7}
                                     & Aggregator & BESSActor & BuildingActor & ChargerActor & DataLogger & UtilityGrid \\ \hline
\multicolumn{1}{|l|}{h1}  & 0          & 0         & 0             & 0            & 1          & 1           \\ \hline
\multicolumn{1}{|l|}{h2}  & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h3}  & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h4}  & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h5}  & 1          & 1        & 0            & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h6}  & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h7}  & 0          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h8}  & 1          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h9}  & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h10} & 0          & 0         & 1             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h11} & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h12} & 0          & 0         & 0             & 0            & 0          & 0           \\ \hline
\end{tabular}
\medskip
\caption{Solver solution for 12 nodes with the basic solver}
\label{tab:basic12node}
\end{table*}

==> tables/mR12node.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{l|l|l|l|l|l|l|}
\cline{2-7}
                                     & Aggregator & BESSActor & BuildingActor & ChargerActor & DataLogger & UtilityGrid \\ \hline
\multicolumn{1}{|l|}{h1}  & 1          & 0         & 1             & 0            & 1          & 1           \\ \hline
\multicolumn{1}{|l|}{h2}  & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h3}  & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h4}  & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h5}  & 1          & 0         & 1             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h6}  & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h7}  & 1          & 1         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h8}  & 1          & 1         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h9}  & 1          & 1         & 0             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h10} & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h11} & 1          & 0         & 1             & 0            & 0          & 0           \\ \hline
\multicolumn{1}{|l|}{h12} & 1          & 0         & 0             & 1            & 0          & 0           \\ \hline
\end{tabular}
\medskip
\caption{Solver solution for 12 nodes with maximum redundancy}
\label{tab:mR12node}
\end{table*}

==> tables/nodetimes.tex <==

\begin{table}[!t]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{No. of nodes} & \textbf{Solution time (s)} \\ \hline
$4$                   & $0.55$                     \\ \hline
$8$                   & $0.62$                     \\ \hline
$12$                  & $0.66$                     \\ \hline
\end{tabular}
\medskip
\caption{Dployment solver timings for different number of nodes}
\label{tab:nodetimes}
\end{table}
